A Biomedical Entity Extraction Pipeline for Oncology Health Records in Portuguese

Textual health records of cancer patients are usually protracted and highly unstructured, making it very time-consuming for health professionals to get a complete overview of the patient's therapeutic course. As such limitations can lead to suboptimal and/or inefficient treatment procedures, healthcare providers would greatly benefit from a system that effectively summarizes the information of those records. With the advent of deep neural models, this objective has been partially attained for English clinical texts, however, the research community still lacks an effective solution for languages with limited resources. In this paper, we present the approach we developed to extract procedures, drugs, and diseases from oncology health records written in European Portuguese. This project was conducted in collaboration with the Portuguese Institute for Oncology which, besides holding over $10$ years of duly protected medical records, also provided oncologist expertise throughout the development of the project. Since there is no annotated corpus for biomedical entity extraction in Portuguese, we also present the strategy we followed in annotating the corpus for the development of the models. The final models, which combined a neural architecture with entity linking, achieved $F_1$ scores of $88.6$, $95.0$, and $55.8$ per cent in the mention extraction of procedures, drugs, and diseases, respectively.

==> tables/data_vertical.tex <==
\begin{table}
\centering
\caption{\label{tab:data} Distribution of the corpus statistics over train, validation, and test sets within the three entity types (procedures, drugs, and diseases). \emph{Sent}, \emph{B}, \emph{I}, and \emph{O} stand for the number of sentences, begin tokens, inside tokens, and outside tokens, respectively.}
\begin{tabular}{llrrrr} 
\toprule
                           &      & \multicolumn{1}{c}{Train} & \multicolumn{1}{c}{Validation} & \multicolumn{1}{c}{Test} & \multicolumn{1}{l}{Total}  \\ 
\midrule
\multirow{4}{*}{Procedure} & Sent & 2,398                     & 599                            & 701                      & 3,698                      \\
                           & B    & 2,091                     & 610                            & 821                      & 3,522                      \\
                           & I    & 1,225                     & 311                            & 452                      & 1,988                      \\
                           & O    & 39,333                    & 8,717                          & 13,992                   & 62,042                     \\ 
\midrule
\multirow{4}{*}{Drug}      & Sent & 1,236                     & 309                            & 377                      & 1,922                      \\
                           & B    & 1,128                     & 285                            & 445                      & 1,858                      \\
                           & I    & 6                         & 2                              & 1                        & 9                          \\
                           & O    & 16,529                    & 4,163                          & 6,737                    & 27,429                     \\ 
\midrule
\multirow{4}{*}{Disease}   & Sent & 1,870                     & 467                            & 608                      & 2,945                      \\
                           & B    & 1,651                     & 395                            & 734                      & 2,780                      \\
                           & I    & 512                       & 141                            & 210                      & 863                        \\
                           & O    & 26,616                    & 5,738                          & 11,743                   & 44,097                     \\
\bottomrule
\end{tabular}
\end{table}
